Continuum Percolation and Stochastic Epidemic Models on Poisson and Ginibre Point Processes

The most studied continuum percolation model in two dimensions is the Boolean model consisting of disks with the same radius whose centers are randomly distributed on the Poisson point process (PPP). We also consider the Boolean percolation model on the Ginibre point process (GPP), which is a typical repelling point process realizing hyperuniformity. We think that the PPP approximates a disordered configuration of individuals, while the GPP does a configuration of citizens adopting a strategy to keep social distancing in a city in order to avoid contagion. We consider the SIR models with contagious infection on supercritical percolation clusters formed on the PPP and the GPP. By numerical simulations, we studied dependence of the percolation phenomena and the infection processes on the PPP- and the GPP-underlying graphs. We show that in a subcritical regime of infection rate the PPP-based models show emergence of infection clusters on clumping of points which is formed by fluctuation of uncorrelated Poissonian statistics. On the other hand, the cumulative numbers of infected individuals in processes are suppressed in the GPP-based models.

==> final/tex/acknowledgement.tex <==
\begin{acknowledgments}
Machiko K. wishes to thank T. J. Kobayashi for carefully reading of the manuscript and useful comments.
This work was supported by
the Grant-in-Aid for Scientific Research (C) (No.19K03674),
(B) (No.18H01124), and
(S) (No.16H06338)
of Japan Society for the Promotion of Science.

\vspace{3mm}
Machiko K. and Makoto K. designed and performed the research and the paper was written cooperatively.
Machiko K. performed computer simulations and data analysis.
\end{acknowledgments}


==> final/tex/references_MK2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%REFERENCES%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thebibliography}{99} 
\bibitem{AM91}
R. M. Anderson and R. M. May,
\textit{Infectious Diseases of Humans:
Dynamics and Control} 
(Oxford University Press, Oxford, 1991)

\bibitem{AFY19}
I. Armend\'ariz, P. A. Ferrari, and S. Yuhjtmanz,
{\sf arXiv:math-ph/1906.11120}

\bibitem{BBA83}
I. Balberg, N. Binenbaum, and C. H. Anderson,
Phys. Rev. Lett. 
\textbf{51}, 1605 (1983)

\bibitem{Bar16}
A.-L. Barab\'asi,
\textit{Network Science}
(Cambridge University Press, Cambridge, 2016)

\bibitem{BY13}
B. B{\l}aszcyszyn and D. Yogeshwarany, 
Elect. J. Probab.
\textbf{18}, no.72, 1 (2013)

\bibitem{BY14}
B. B{\l}aszcyszyn and D. Yogeshwarany, 
Adv. Appl. Prob. (SGSA)
\textbf{46}, 1 (2014)

\bibitem{BR06}
B. Bollobas and O. Riordan,
\textit{Percolation}
(Cambridge University Press, Cambridge, 2006)

\bibitem{CHBC09}
G. Chowell, J. M. Hyman, L. M. A. Bettencourt, and
C. Castillo-Chavez (ed.),
\textit{Mathematical and Statistical Estimation 
Approach in Epidemiology}
(Springer, Dordrecht, 2009)

\bibitem{DVJ03}
D. J. Daley and D. Vere-Jones,
\textit{An Introduction to the Theory of Point Processes},
Vol. i, 2nd ed.
(Springer, New York, 2003)

\bibitem{DH00}
O. Diekmann and J. A. P. Heesterbeck,
\textit{Mathematical Epidemiology of Infectious Diseases:
Model Building, Analysis and Interpretation}
(John Wiley and Sons, Chichester, 2000)

\bibitem{EC20}
R. Erban and S. J. Chapman,
\textit{Stochastic Modeling of Reaction-Diffusion Processes}
(Cambridge University Press, Cambridge, 2020)

\bibitem{For10}
P. J. Forrester, 
\textit{Log-gases and Random Matrices}
(Princeton University Press, Princeton, NJ, 2010)

\bibitem{GS81}
E. T. Gawlinski and H. E. Stanley,
J. Phys. A: Math. Gen.
\textbf{14}, L291 (1981)

\bibitem{GKP16}
S. Ghosh, M. Krishnapur, and Y. Peres, 
Ann. Probab. 
\textbf{44}, 3357 (2016)

\bibitem{Gilb61}
E. N. Gilbert,
J. Soc. Indust. Appl. Math.
\textbf{9}, 533 (1961)

\bibitem{Gil76}
D. Gillespie,
J. Comput. Phys.
\textbf{22}, 403 (1976)

\bibitem{Gil77}
D. Gillespie,
J. Phys. Chem.
\textbf{81}, 2340 (1977)

\bibitem{Gin65}
J. Ginibre, 
J. Math. Phys.
\textbf{6}, 440 (1965)

\bibitem{Hin00}
H. Hinrichsen,
Adv. Phys.
\textbf{49}, 815 (2000)

\bibitem{HKPV09}
J. B., Hough, M. Krishnapur, Y. Peres, and B. Vir\'ag, 
\textit{
Zeros of Gaussian Analytic Functions
and Determinantal Point Processes} 
(Providence, RI : Amer. Math. Soc., 2009)

\bibitem{Kat15}
M. Katori, 
\textit{Bessel Processes, Schramm--Loewner Evolution
and the Dyson Model}
(Springer, Tokyo, 2015)

\bibitem{LBDA15}
Y. Li, F. Baccelli, H. S. Dhillon, and J. G. Andrews,
IEEE Trans. Cpmmin. 
\textbf{63}, 3405 (2015)

\bibitem{Lig85}
T. Liggett,
\textit{Interacting Particle Systems}
(Springer, New York, 1985). 

\bibitem{Lig99}
T. Liggett,
\textit{Stochastic Interacting Systems:
Contact, Voter and Exclusion Processes}
(Springer, New York, 1999). 

\bibitem{MKS21}
T. Matsui, M. Katori, and T. Shirai, 
to apear in J. Phys. A: Math. Theor. 
{\sf arXiv:math.PR/2012.10585}

\bibitem{Meh04}
M. L. Mehta, 
\textit{Random Matrices}, 3rd edn
(Elsevier/Academic Press, Amsterdam, 2004) 

\bibitem{MM12}
S. Mertens and C. Moore,
Phys. Rev. E 
\textbf{86}, 061109 (2012)

\bibitem{MR96}
R. Meester and R. Roy,
\textit{Continuum Percolation}
(Cambridge University Press, Cambridge, 1996)

\bibitem{MS14}
N. Miyoshi and T. Shirai,
Adv. Appl. Probab.
\textbf{46}, 832 (2014)

\bibitem{MS16}
N. Miyoshi and T. Shirai,
IEICE Trans. Commun.
\textbf{E99-B}, 2247 (2016)

\bibitem{NZ01}
M. E. J. Newman and R. M. Ziff,
Phys. Rev. E
\textbf{64}, 016706 (2001)

\bibitem{QT99}
J. Quintanilla and S. Torquato,
J. Chem. Phys.
\textbf{111}, 5947 (1999)

\bibitem{QTZ00}
J. Quintanilla, S. Torquato, and R. M. Ziff,
J. Phys. A: Math. Gen. 
\textbf{33}, L399 (2000)

\bibitem{QZ07}
J. A. Quintanilla and R. M. Ziff,
Phys. Rev. E
\textbf{76}, 051115 (2007)

\bibitem{SMDHB20}
S. Saha, A. Mishra, S. K. Dana, C. Hens, and N. Bairagi, 
Phys. Rev. E
\textbf{102}, 052307 (2020)

\bibitem{SN21}
H. Sakaguchi and Y. Nakao,
Phys. Rev. E
\textbf{103}, 012301 (2021)

\bibitem{SAAMF20}
G. B. M. Santosa, T. F. A. Alvesa, G. A. Alvesb, 
A. Macedo-Filhoc, and R. S. Ferreirad, 
Phys. Lett. A
\textbf{384}, 126063 (2020)

\bibitem{Shi06}
T. Shirai, 
J. Stat. Phys. 
\textbf{123}, 615 (2006)

\bibitem{ST03a}
T. Shirai and Y. Takahashi, 
J. Funct. Anal.
\textbf{205}, 414 (2003)

\bibitem{ST03b}
T. Shirai and Y. Takahashi, 
Ann. Probab.
\textbf{31}, 1533 (2003)

\bibitem{Sos00}
A. Soshnikov,
Russian Math. Surveys
\textbf{55}, 923 (2000)

\bibitem{SA92}
D. Stauffer and A. Aharony,
\textit{Introduction to Percolation Theory}
(Taylor \& Francis, London, 1992)

\bibitem{TI06}
H. Tamura and K. R. Ito,
Commun. Math. Phys.
Commun. Math. Phys.
\textbf{263}, 353 (2006)

\bibitem{TI07}
H. Tamura and K. R. Ito,
J. Func. Anal.
\textbf{243}, 207 (2007)

\bibitem{TZ10}
T. Tom\'e and R. M. Ziff,
Phys. Rev. E
\textbf{82}, 051921 (2010)

\bibitem{Tor18}
S. Torquato, 
Phys. Rep. 
\textbf{745}, 1 (2018)

\bibitem{VFM09}
T. Vojta, A. Farquhar, and J. Mast,
Phys. Rev. E
\textbf{79}, 011111 (2009)

\end{thebibliography}
